Probabilistic PolarGMM: Unsupervised Cluster Learning of Very Noisy Projection Images of Unknown Pose

A crucial step in single particle analysis (SPA) of cryogenic electron microscopy (Cryo-EM), 2D classification and alignment takes a collection of noisy particle images to infer orientations and group similar images together. Averaging these aligned and clustered noisy images produces a set of clean images, ready for further analysis such as 3D reconstruction. Fourier-Bessel steerable principal component analysis (FBsPCA) enables an efficient, adaptable, low-rank rotation operator. We extend the FBsPCA to additionally handle translations. In this extended FBsPCA representation, we use a probabilistic polar-coordinate Gaussian mixture model to learn soft clusters in an unsupervised fashion using an expectation maximization (EM) algorithm. The obtained rotational clusters are thus additionally robust to the presence of pairwise alignment imperfections. Multiple benchmarks from simulated Cryo-EM datasets show probabilistic PolarGMM's improved performance in comparisons with standard single-particle Cryo-EM tools, EMAN2 and RELION, in terms of various clustering metrics and alignment errors.

==> sections/04_analysis.tex <==
\section{Analysis of FBsPCA}
\label{Section:Analysis:Algorithms}

In this section, we provide a justification that the GMM described above is suitable to recover the underlying cluster structures using the output of the FBsPCA. 

To this end, we consider the following noise model for generating the input images. Suppose there are $K$ image clusters $\set{C}_i, i \in [K]$. Each cluster $N$ images. We model each cluster as samples from an underlying Gaussian distribution $(\bs{c}_i, \Lambda_i)$, where $\bs{c}_i$ is the cluster center, and $\Lambda_i$ is the covariance matrix. To model the rotational variation, we generate each input image $I_{ij}, i\in [K], j \in [N]$ by an angle $\alpha_{ij}$, from which we then impose the element-wise noise specified by $\Lambda_i$. In this analysis, we assume $\Lambda_i = \sigma^2 I_{n^2}$. 

To ease our discussion, let us define the $k$-th order Fourier Bessel transform in the matrix form:
\begin{definition}
Denote $A^{(k)}: \calR^{n\times n} \rightarrow \calC^{q_k}$ as the linear transformation that takes an input image and outputs its $k$-th order complex coefficients. Note that this map is independent of specific images. 
\end{definition}

The following proposition states that $A_k$ is a unitary matrix.
\begin{proposition}
$A^{(k)}$ is a complex unitary matrix, i.e., 
\begin{equation}
{\overline{A}^{(k)}}^T \cdot A^{(k)} = I_{q_k}.
\label{Eq:A:k:Orthogonal}
\end{equation}
\end{proposition}

\begin{proof}
Note that the $q$-th column of $A^{(k)}$ corresponds to the following operator:
\begin{equation}
A^{(k)}_q(I) := \int_{0}^{\gamma}\big(\int_{0}^{2\pi} I\cdot \psi^{k,q}(r,\phi)d\phi\big)dr.
\label{Eq:Mat:A}
\end{equation}
Therefore,
\begin{align*}
& \bs{e}_q^T\big({\overline{A}^{(k)}}^T \cdot A^{(k)}\big)\bs{e}_{q'} \\
= & \int_{0}^{\gamma}\big(\int_{0}^{2\pi} \psi^{k,q'}(r,\phi) \cdot \psi^{k,q}(r,\phi)d\phi\big)dr \\
= & \delta_{q,q'}
\end{align*}
which ends the proof.
\end{proof}

Denote $I_{ij} = R(\alpha_{ij})\bs{c}_i + \epsilon_{ij}$, where $R(\alpha_{ij})$ denotes the rotational operator, and where $\epsilon_{ij}$ denotes the image noise. We can calculate the covariance matrix as follows:


The covariance matrix becomes
\begin{align*}
\Sigma_k & = \frac{1}{KN}\sum\limits_{i=1}^{K}\sum\limits_{j=1}^{N} Re\Big(\big(A_k(\bs{c}_i)\cdot e^{-i\cdot k \alpha_{ij}} + A_k(\epsilon_{ij})\big)\cdot\big( \overline{A_k(\bs{c}_i)}^T\cdot e^{i\cdot k \alpha_{ij}} + \overline{A_k(\epsilon_{ij})}^T\big)\Big) \\
&= \frac{1}{KN}\sum\limits_{i=1}^{K}\sum\limits_{j=1}^{N} Re\big(A_k(\bs{c}_i)\cdot \overline{A_k(\bs{c}_i)}^T\big) \\
& \quad + \frac{1}{KN}\sum\limits_{i=1}^{K}\sum\limits_{j=1}^{N}Re\big(A_{k}(\epsilon_{ij})\cdot \overline{A_{k}(\bs{c}_i)}^T e^{ik\alpha_{ij}} + A_{k}(\bs{c}_i)\cdot e^{-i k \alpha_{ij}}\overline{A_{k}(\epsilon_{ij})}^T+A_{k}(\epsilon_{ij})\cdot \overline{A_{k}(\epsilon_{ij})}^T\big) \\
&= \frac{1}{K}\sum\limits_{i=1}^{K} Re\big(\set{A}_k(\bs{c}_i)\cdot \overline{\set{A}_k(\bs{c}_i)}^T+A_{k}(\frac{1}{N}\sum\limits_{j=1}^{N} \epsilon_{ij} \cdot \overline{\bs{c}}_i\cdot e^{ik \alpha_{ij}} + \bs{c}_i\cdot e^{-ik\alpha_{ij}}\overline{\epsilon}_{ij}^T +\epsilon_{ij}\cdot \overline{\epsilon}_{ij}^T)\overline{A}_k\big)
\end{align*}

In other words, we can view $\Sigma_k$ as a perturbation from the underlying covariance matrix $\frac{1}{K}\sum\limits_{i=1}^{K} Re\big(\set{A}_k(\bs{c}_i)\cdot \overline{\set{A}_k(\bs{c}_i)}^T\big)$. In the following, we use stability of leading eigen-spaces to show that if the clusters are well seperated in the original space, then they are seperated in the embedded space. 

We first characterize the spectrum of the ground-truth covariance matrix which is given by
\begin{equation}
\Sigma_k^{\gt} = A_k (\frac{1}{K}\sum\limits_{i=1}^{K}\bs{c}_i \bs{c}_i^T)\overline{A}_k.
\end{equation}

Let the eigenvalues of $C = \frac{1}{K}\sum\limits_{i=1}^{K}\bs{c}_i \bs{c}_i^T$ in the decreasing order as $\mu_1\geq \mu_2\geq \cdots \mu_{K}\geq \mu_{K+1} = 0$. 

\begin{definition}
We say underlying cluster centers $\bs{c}_i, i \in [K]$ are $(\delta_{\min}, \delta_{\max})$-regular if
\begin{equation}
\delta_{\min} U U^T\preceq \frac{1}{K}\sum\limits_{k=1}^{K}\bs{c}_i\bs{c}_i^T \preceq \delta_{\max} U U^T,     
\end{equation}
where $U \in \R^{n^2\times K}$ is an orthonormal basis of the linear space spanned by $\bs{c}_i, i \in [K]$.
\end{definition}

\begin{definition}
We define the maximum angle $\sigma(A_k, U)$ between $A_k$ and $U$ as the minimum singular value of $(Re(A_k), Im(A_k))(U,0;0,U)$. 
\end{definition}

\begin{proposition}
If $\bs{c}_i, i \in [K]$ are $(\delta_{\min},\delta_{\max})$-regular, then there exists an orthogonal matrix $\overline{U}\in \R^{q_k\times K}$ so that
\begin{equation}
\delta_{\min}\cdot \sigma(A_k,U) \overline{U}\overline{U}^T \preceq Re(A_k (\frac{1}{K}\sum\limits_{i=1}^{K}\bs{c}_i\bs{c}_i^T)\overline{A}_k^T)
\end{equation}
\end{proposition}

Denote
\begin{equation}
E = \frac{1}{K}Re\Big(\sum\limits_{i=1}^{K}\sum\limits_{j=1}^{N} A_k\big(\frac{1}{N}\sum\limits_{j=1}^{N}\epsilon_{ij}\cdot \bs{c}_i\cdot e^{ik\alpha_{ij}} + \bs{c}_i\cdot e^{-ik\alpha_{ij}}\epsilon_{ij}^T + \epsilon_{ij}\epsilon_{ij}^T\big)\overline{A}_k^T\Big).
\end{equation}

We need to analyze the concentration properties for the following quantities:
\begin{align*}
f_1 & = \frac{1}{KN}\sum\limits_{i=1}^{K}\sum\limits_{j=1}^{N} Re(A_k)\epsilon_{ij}\cdot \bs{b}_{ij}^T \qquad \bs{b}_{ij}:= \cos(k\alpha_{ij})(A_k\bs{c}_i) + \sin(k\alpha_{ij})(B_k\bs{c}_i)\\
f_2 & = \frac{1}{KN}\sum\limits_{i=1}^{K}\sum\limits_{i=1}^{N} Im(A_k)\epsilon_{ij}\cdot \bs{a}_{ij}^T\qquad \bs{a}_{ij}:= \cos(k\alpha_{ij})(B_k \bs{c}_i) - \sin(k\alpha_{ij})(A_k \bs{c}_i) \\
f_3 &= Re\Big(A_k\big(\frac{1}{KN}\sum\limits_{i=1}^{K}\sum\limits_{j=1}^{N}\epsilon_{ij}\epsilon_{ij}^T\big)\overline{A}_k\Big) 
\end{align*}

$f_1$ and $f_2$ are similar, and their concentration bounds 

\begin{lem}
Consider $n$ independent Gaussian random variables $\epsilon_i \in \set{N}(0,I_m), i\in [n]$ and vectors $\bs{b}_i \in \R^{q}, i\in [n]$. Given a matrix $A\in R^{q\times m}$. Then we have 
\begin{equation}
Pr[\|Z\|\geq t]\leq \max(m,q) exp\big(-\frac{t^2}{2L}\big), \qquad Z:= \sum\limits_{i=1}^n A \epsilon_i \bs{b}_i^T.
\label{Eq:Random:Concentration0}
\end{equation}
where
$$
L:= \max\big(Tr(A^TA)\|\sum\limits_{i=1}^n \bs{b}_i\bs{b}_i^T\|,(\sum\limits_{i=1}^n\|\bs{b}_i\|^2)\|AA^T\|\big).
$$
\end{lem}

\begin{proof}
The proof of this relies on bounding
$$
E[Tr((ZZ^T)^{2k})].
$$
\end{proof}


$f_3$ is the generalized chi-square random variable and satisfies the following lemma.
\begin{lem}
Suppose $\epsilon_{ij}$ are independent random variables following the normal distribution $\set{N}(0,\sigma^2I_n)$, then 
\begin{equation}
Pr\big(\|\frac{1}{KN}\sum\limits_{i=1}^{K}\sum\limits_{j=1}^{N}\epsilon_{ij}\epsilon_{ij}^T-\sigma^2 I_{n^2}\|\geq t\sigma^2\big) \leq \exp (-\frac{KN t^2}{8}).
\label{Eq:Random:Concentration}
\end{equation}
\end{lem}

We can use the standard Davis-Kham theorem to bound the projections defined by the leading eigenspaces of two matrices, where one is the perturbation of another. 
\begin{lem}
[DK70]. Given two matrices $A\in \R^{q\times q}$ and $A+E\in \R^{q\times q}$. Let $U\in \R^{L\times q}$ and $\overline{U}\in \R^{L\times q}$ be the leading eigenspace of $A$ and $A+E$, respectively. Let $\lambda_1(A)\geq \lambda_2(A)\geq \cdots \geq \lambda_L(A)>\lambda_{L+1}(A)$ be the eigenvalues of $A$ in the decreasing order. Suppose $\|E\| < \lambda_L(A)-\lambda_{L+1}(A)$, then 
\begin{equation}
d(U, \overline{U})\leq \frac{\|E\|}{\lambda_{L}(A)-\lambda_{L+1}(A)-\|E\|}.
\label{Eq:Stability:BoUND}    
\end{equation}
where $d(U,\overline{U})$ denotes the distance between $U$ and $\overline{U}$.
\end{lem}

\begin{remark}
Note that $d(U,\overline{U})$ controls many geometric quantities provided by $U$ and $\overline{U}$, including the projection distances between vectors produced by $U$ and $\overline{U}$, which are what we need. 
\end{remark}

